Contrastive Language-Action Pre-training for Temporal Localization

Long-form video understanding requires designing approaches that are able to temporally localize activities or language. End-to-end training for such tasks is limited by the compute device memory constraints and lack of temporal annotations at large-scale. These limitations can be addressed by pre-training on large datasets of temporally trimmed videos supervised by class annotations. Once the video encoder is pre-trained, it is common practice to freeze it during fine-tuning. Therefore, the video encoder does not learn temporal boundaries and unseen classes, causing a domain gap with respect to the downstream tasks. Moreover, using temporally trimmed videos prevents to capture the relations between different action categories and the background context in a video clip which results in limited generalization capacity. To address these limitations, we propose a novel post-pre-training approach without freezing the video encoder which leverages language. We introduce a masked contrastive learning loss to capture visio-linguistic relations between activities, background video clips and language in the form of captions. Our experiments show that the proposed approach improves the state-of-the-art on temporal action localization, few-shot temporal action localization, and video language grounding tasks.

==> tables/FewShotTAL_main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!t]
\centering
%\scriptsize
\small
\resizebox{0.7\linewidth}{!}{    
\begin{tabular}{l|c|c|c|c|c}
\hline    
       & \textbf{Pre-train} &   \multicolumn{3}{c|}{\textbf{mAP, tIoU@X } }& \textbf{Avg.} \\ 
      & \textbf{Dataset} & \textbf{0.5} & \textbf{0.75} & \textbf{0.95} & \textbf{mAP} \\ \hline
QAT~\cite{nag2021fewshot}                     & K400                         & 65.25                 & 37.60                   & 3.74                   & 37.37             \\ \hline
TAC~\cite{tran2018closer}& ANET-160                     & 65.94                 & 38.61                  & 3.31                   & 38.06             \\ 
TSP~\cite{alwassel_2021_tsp} & ANET-160                     & 67.73                 & 38.62                  & 4.71                   & 38.7              \\ \hline 
%Placeholder             &                              &                       &                        &                        &                   \\ \hline
CLAP$^{(clip)}$ & ANET-160                     & 65.75                 & 38.93                  & \textbf{6.85}                   & 39.07             \\ 
CLAP$^{(mask)}$            & ANET-160                     & 67.12                     & 39.59                      & 6.00                      & 39.32                 \\ 
CLAP         & ANET-160                     & \textbf{67.58                   } & \textbf{39.77}                      & 6.62                      & \textbf{40.25}            \\ \hline    
\end{tabular}
}
\caption{
\textbf{Results for few-shot TAL on ActivityNet-1.3 using QAT~\cite{nag2021fewshot} with different pre-training strategies.} 
We report the mAP at different tIoU thresholds and the average mAP.
We denote with $^{(\cdot)}$ the method which uses only language templates.
}
\label{tab:TAL_fewshot}
\end{table}
			

